Private Information Retrieval for Large-Scale DNA-Based Data Storage

We investigate Private Information Retrieval (PIR) in the context of synthetic DNA-based data storage. While PIR is a well-studied primitive for digital databases, extending it to DNA-based databases presents unique challenges arising from biochemical query mechanisms and their complexity. We propose two approaches for adapting two-server PIR protocols to DNA-based storage, balancing privacy, efficiency, and feasibility. These approaches illustrate how information-theoretic privacy trade-offs manifest in DNA-based storage systems.

==> aux/packages.tex <==
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{ifthen}
\makeatletter
\@ifclassloaded{sn-jnl}{%
    % sn-jnl.cls already loads url, amsthm, hyperref and natbib (which replaces cite)
    \usepackage{amsmath}
}{\@ifclassloaded{beamer}{%
    % slides: beamer has its own citation and theorem handling
    \usepackage{amsmath}
    \providecommand{\qedsymbol}{} % redefined in macros.tex
}{%
    \usepackage{url}
    \usepackage{cite}
    \usepackage[cmex10]{amsmath}
    \usepackage{amsthm}
}}
\makeatother
\usepackage{amssymb}
\usepackage{bbm}
\usepackage{bm}
\usepackage{comment}
\usepackage{dirtytalk}
\usepackage{graphicx}
\usepackage{xcolor}
\usepackage{soul}

% Everything below is for the paper versions only (enumitem breaks beamer's lists)
\makeatletter
\@ifclassloaded{beamer}{}{%
    \usepackage{balance}
    \usepackage[ruled, linesnumbered, vlined]{algorithm2e}
    \usepackage{enumitem}
    \usepackage[capitalize]{cleveref}

    \@ifclassloaded{sn-jnl}{\theoremstyle{thmstyleone}}{} % theorem styles of sn-jnl.cls
    \newtheorem{corollary}{Corollary}
    \newtheorem{proposition}{Proposition}
    \newtheorem{lemma}{Lemma}
    \newtheorem{theorem}{Theorem}
    \@ifclassloaded{sn-jnl}{\theoremstyle{thmstyletwo}}{}
    \newtheorem{remark}{Remark}
}
\makeatother

